MMAD-Purify: A Precision-Optimized Framework for Efficient and Scalable Multi-Modal Attacks

Neural networks have achieved remarkable performance across a wide range of tasks, yet they remain susceptible to adversarial perturbations, which pose significant risks in safety-critical applications. With the rise of multimodality, diffusion models have emerged as powerful tools not only for generative tasks but also for various applications such as image editing, inpainting, and super-resolution. However, these models still lack robustness due to limited research on attacking them to enhance their resilience. Traditional attack techniques, such as gradient-based adversarial attacks and diffusion model-based methods, are hindered by computational inefficiencies and scalability issues due to their iterative nature. To address these challenges, we introduce an innovative framework that leverages the distilled backbone of diffusion models and incorporates a precision-optimized noise predictor to enhance the effectiveness of our attack framework. This approach not only enhances the attack's potency but also significantly reduces computational costs. Our framework provides a cutting-edge solution for multi-modal adversarial attacks, ensuring reduced latency and the generation of high-fidelity adversarial examples with superior success rates. Furthermore, we demonstrate that our framework achieves outstanding transferability and robustness against purification defenses, outperforming existing gradient-based attack models in both effectiveness and efficiency.

==> ablation-all.tex <==
\begin{table*}[ht]
    \centering
    \resizebox{0.49\linewidth}{!}{%
\begin{tabular}{cccccccccccc}
\hline
\multicolumn{2}{c}{}                                                    & \multicolumn{6}{c}{neural networks}                                                                                                                                                                                                                                   & \multicolumn{4}{c}{IQAs}                                                                                       \\
\multicolumn{2}{c}{\multirow{-2}{*}{$\epsilon$}}                        & VGG19                                 & RN50                                                          & WR101                                 & DN121                                 & NNv2                                  & SNv2                                  & PSNR $\uparrow$              & SSIM $\uparrow$             & FID $\downarrow$             & LPIPS $\downarrow$ \\ \hline
\multicolumn{1}{c}{}                         & \multicolumn{1}{c|}{8}  & \multicolumn{1}{c|}{54.83\%}          & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}46.39\%}          & \multicolumn{1}{c|}{41.79\%}          & \multicolumn{1}{c|}{47.06\%}          & \multicolumn{1}{c|}{54.96\%}          & \multicolumn{1}{c|}{\hl{61.82\%}} & \multicolumn{1}{c|}{28.5718} & \multicolumn{1}{c|}{0.839}  & \multicolumn{1}{c|}{16.0097} & 0.1743             \\
\multicolumn{1}{c}{\multirow{-2}{*}{$p_1$}}  & \multicolumn{1}{c|}{16} & \multicolumn{1}{c|}{\hl{58.76\%}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\hl{69.50\%}} & \multicolumn{1}{c|}{\hl{46.67\%}} & \multicolumn{1}{c|}{\hl{49.77\%}} & \multicolumn{1}{c|}{\hl{58.80\%}} & \multicolumn{1}{c|}{60.45\%}          & \multicolumn{1}{c|}{28.2141} & \multicolumn{1}{c|}{0.8194} & \multicolumn{1}{c|}{19.1739} & 0.1964             \\ \hline
\multicolumn{1}{c}{}                         & \multicolumn{1}{c|}{8}  & \multicolumn{1}{c|}{\hl{51.13\%}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}32.48\%}          & \multicolumn{1}{c|}{\hl{38.81\%}} & \multicolumn{1}{c|}{\hl{43.92\%}} & \multicolumn{1}{c|}{\hl{50.20\%}} & \multicolumn{1}{c|}{\hl{60.52\%}} & \multicolumn{1}{c|}{27.2604} & \multicolumn{1}{c|}{0.8046} & \multicolumn{1}{c|}{19.7477} & 0.2008             \\
\multicolumn{1}{c}{\multirow{-2}{*}{$p_1+$}} & \multicolumn{1}{c|}{16} & \multicolumn{1}{c|}{49.68\%}          & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\hl{44.52\%}} & \multicolumn{1}{c|}{36.04\%}          & \multicolumn{1}{c|}{41.27\%}          & \multicolumn{1}{c|}{50.08\%}          & \multicolumn{1}{c|}{53.31\%}          & \multicolumn{1}{c|}{27.1135} & \multicolumn{1}{c|}{0.7968} & \multicolumn{1}{c|}{20.9897} & 0.2049             \\ \hline
\multicolumn{1}{c}{}                         & \multicolumn{1}{c|}{8}  & \multicolumn{1}{c|}{\hl{80.49\%}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}89.92\%}          & \multicolumn{1}{c|}{69.90\%}          & \multicolumn{1}{c|}{72.55\%}          & \multicolumn{1}{c|}{79.37\%}          & \multicolumn{1}{c|}{77.22\%}          & \multicolumn{1}{c|}{26.8757} & \multicolumn{1}{c|}{0.8189} & \multicolumn{1}{c|}{31.0186} & 0.2237             \\
\multicolumn{1}{c}{\multirow{-2}{*}{$p_2$}}  & \multicolumn{1}{c|}{16} & \multicolumn{1}{c|}{80.25\%}          & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\hl{95.50\%}} & \multicolumn{1}{c|}{\hl{75.68\%}} & \multicolumn{1}{c|}{\hl{73.60\%}} & \multicolumn{1}{c|}{\hl{80.13\%}} & \multicolumn{1}{c|}{\hl{75.61\%}} & \multicolumn{1}{c|}{26.4921} & \multicolumn{1}{c|}{0.797}  & \multicolumn{1}{c|}{36.2468} & 0.2549             \\ \hline
\multicolumn{1}{c}{}                         & \multicolumn{1}{c|}{8}  & \multicolumn{1}{c|}{\hl{76.39\%}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}80.57\%}          & \multicolumn{1}{c|}{66.17\%}          & \multicolumn{1}{c|}{67.45\%}          & \multicolumn{1}{c|}{79.17\%}          & \multicolumn{1}{c|}{\hl{72.89\%}} & \multicolumn{1}{c|}{24.9906} & \multicolumn{1}{c|}{0.7804} & \multicolumn{1}{c|}{40.5354} & 0.2662             \\
\multicolumn{1}{c}{\multirow{-2}{*}{$p_2+$}} & \multicolumn{1}{c|}{16} & \multicolumn{1}{c|}{76.27\%}          & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\hl{88.95\%}} & \multicolumn{1}{c|}{\hl{72.97\%}} & \multicolumn{1}{c|}{\hl{70.71\%}} & \multicolumn{1}{c|}{\hl{79.81\%}} & \multicolumn{1}{c|}{73.17\%}          & \multicolumn{1}{c|}{24.7144} & \multicolumn{1}{c|}{0.7628} & \multicolumn{1}{c|}{44.6224} & 0.2906             \\ \hline
\end{tabular}%
}
\hfill
\resizebox{0.49\linewidth}{!}{%
\begin{tabular}{cccccccccccc}
\hline
\multicolumn{2}{c}{}                                                    & \multicolumn{6}{c}{neural networks}                                                                                                                                                                                                                                   & \multicolumn{4}{c}{IQAs}                                                                                       \\
\multicolumn{2}{c}{\multirow{-2}{*}{$I$}}                      & VGG19                                 & RN50                                                          & WR101                                 & DN121                                 & NNv2                                  & SNv2                                  & PSNR $\uparrow$              & SSIM $\uparrow$             & FID $\downarrow$             & LPIPS $\downarrow$ \\ \hline
\multicolumn{1}{c}{}                         & \multicolumn{1}{c|}{8}  & \multicolumn{1}{c|}{55.99\%}          & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}59.79\%}          & \multicolumn{1}{c|}{44.42\%}          & \multicolumn{1}{c|}{48.76\%}          & \multicolumn{1}{c|}{58.08\%}          & \multicolumn{1}{c|}{59.61\%}          & \multicolumn{1}{c|}{28.3865} & \multicolumn{1}{c|}{0.8297} & \multicolumn{1}{c|}{17.3677} & 0.1841             \\
\multicolumn{1}{c}{\multirow{-2}{*}{$p_1$}}  & \multicolumn{1}{c|}{10} & \multicolumn{1}{c|}{\hl{58.76\%}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\hl{69.50\%}} & \multicolumn{1}{c|}{\hl{46.67\%}} & \multicolumn{1}{c|}{\hl{49.77\%}} & \multicolumn{1}{c|}{\hl{58.80\%}} & \multicolumn{1}{c|}{\hl{60.45\%}} & \multicolumn{1}{c|}{28.2141} & \multicolumn{1}{c|}{0.8194} & \multicolumn{1}{c|}{19.1739} & 0.1964             \\ \hline
\multicolumn{1}{c}{}                         & \multicolumn{1}{c|}{8}  & \multicolumn{1}{c|}{\hl{51.23\%}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}41.35\%}          & \multicolumn{1}{c|}{35.74\%}          & \multicolumn{1}{c|}{\hl{44.61\%}} & \multicolumn{1}{c|}{\hl{50.09\%}} & \multicolumn{1}{c|}{\hl{54.76\%}} & \multicolumn{1}{c|}{27.1838} & \multicolumn{1}{c|}{0.8007} & \multicolumn{1}{c|}{20.216}  & 0.2023             \\
\multicolumn{1}{c}{\multirow{-2}{*}{$p_1+$}} & \multicolumn{1}{c|}{10} & \multicolumn{1}{c|}{49.68\%}          & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\hl{44.52\%}} & \multicolumn{1}{c|}{\hl{36.04\%}} & \multicolumn{1}{c|}{41.27\%}          & \multicolumn{1}{c|}{50.08\%}          & \multicolumn{1}{c|}{53.31\%}          & \multicolumn{1}{c|}{27.1135} & \multicolumn{1}{c|}{0.7968} & \multicolumn{1}{c|}{20.9897} & 0.2049             \\ \hline
\multicolumn{1}{c}{}                         & \multicolumn{1}{c|}{8}  & \multicolumn{1}{c|}{\hl{81.16\%}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}93.85\%}          & \multicolumn{1}{c|}{75.41\%}          & \multicolumn{1}{c|}{\hl{75.62\%}} & \multicolumn{1}{c|}{\hl{80.46\%}} & \multicolumn{1}{c|}{\hl{76.70\%}} & \multicolumn{1}{c|}{26.6618} & \multicolumn{1}{c|}{0.8066} & \multicolumn{1}{c|}{33.906}  & 0.2409             \\
\multicolumn{1}{c}{\multirow{-2}{*}{$p_2$}}  & \multicolumn{1}{c|}{10} & \multicolumn{1}{c|}{80.25\%}          & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\hl{95.50\%}} & \multicolumn{1}{c|}{\hl{75.68\%}} & \multicolumn{1}{c|}{73.60\%}          & \multicolumn{1}{c|}{80.13\%}          & \multicolumn{1}{c|}{75.61\%}          & \multicolumn{1}{c|}{26.4921} & \multicolumn{1}{c|}{0.797}  & \multicolumn{1}{c|}{36.2468} & 0.2549             \\ \hline
\multicolumn{1}{c}{}                         & \multicolumn{1}{c|}{8}  & \multicolumn{1}{c|}{75.53\%}          & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}84.48\%}          & \multicolumn{1}{c|}{67.98\%}          & \multicolumn{1}{c|}{69.65\%}          & \multicolumn{1}{c|}{\hl{81.71\%}} & \multicolumn{1}{c|}{72.62\%}          & \multicolumn{1}{c|}{24.8471} & \multicolumn{1}{c|}{0.7705} & \multicolumn{1}{c|}{43.1882} & 0.2798             \\
\multicolumn{1}{c}{\multirow{-2}{*}{$p_2+$}} & \multicolumn{1}{c|}{10} & \multicolumn{1}{c|}{\hl{76.27\%}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\hl{88.95\%}} & \multicolumn{1}{c|}{\hl{72.97\%}} & \multicolumn{1}{c|}{\hl{70.71\%}} & \multicolumn{1}{c|}{79.81\%}          & \multicolumn{1}{c|}{\hl{73.17\%}} & \multicolumn{1}{c|}{24.7144} & \multicolumn{1}{c|}{0.7628} & \multicolumn{1}{c|}{44.6224} & 0.2906             \\ \hline
\end{tabular}%
}\\
\vspace{0.5em}
\resizebox{0.49\linewidth}{!}{%
\begin{tabular}{cccccccccccc}
\hline
\multicolumn{2}{c}{}                               & \multicolumn{6}{c}{neural networks}                                                                                                                                                                                                                                     & \multicolumn{4}{c}{IQAs}                                                                                                                  \\
\multicolumn{2}{c}{\multirow{-2}{*}{$L$}} & VGG19                                  & RN50                                                          & WR101                                 & DN121                                 & NNv2                                   & SNv2                                  & PSNR $\uparrow$                       & SSIM $\uparrow$                      & FID $\downarrow$                      & LPIPS $\downarrow$ \\ \hline
                         & \multicolumn{1}{c|}{1}  & \multicolumn{1}{c|}{\hl{68.80\%}}  & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}62.11\%}          & \multicolumn{1}{c|}{\hl{55.05\%}} & \multicolumn{1}{c|}{\hl{62.50\%}} & \multicolumn{1}{c|}{\hl{59.51\%}}  & \multicolumn{1}{c|}{57.73\%}          & \multicolumn{1}{c|}{\hl{28.4538}} & \multicolumn{1}{c|}{\hl{0.8313}} & \multicolumn{1}{c|}{\hl{13.7087}} & \hl{0.1774}    \\
                         & \multicolumn{1}{c|}{5}  & \multicolumn{1}{c|}{60.36\%}           & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}52.99\%}          & \multicolumn{1}{c|}{40.17\%}          & \multicolumn{1}{c|}{47.25\%}          & \multicolumn{1}{c|}{57.77\%}           & \multicolumn{1}{c|}{60.23\%}          & \multicolumn{1}{c|}{28.367}           & \multicolumn{1}{c|}{0.8266}          & \multicolumn{1}{c|}{17.6228}          & 0.1877             \\
                         & \multicolumn{1}{c|}{10} & \multicolumn{1}{c|}{58.76\%}           & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\hl{69.50\%}} & \multicolumn{1}{c|}{46.67\%}          & \multicolumn{1}{c|}{49.77\%}          & \multicolumn{1}{c|}{58.80\%}           & \multicolumn{1}{c|}{\hl{60.45\%}} & \multicolumn{1}{c|}{28.2141}          & \multicolumn{1}{c|}{0.8194}          & \multicolumn{1}{c|}{19.1739}          & 0.1964             \\
\multirow{-4}{*}{$p_1$}  & \multicolumn{1}{c|}{20} & \multicolumn{1}{c|}{57.64\%}           & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}67.45\%}          & \multicolumn{1}{c|}{44.93\%}          & \multicolumn{1}{c|}{52.49\%}          & \multicolumn{1}{c|}{55.84\%}           & \multicolumn{1}{c|}{59.51\%}          & \multicolumn{1}{c|}{28.2208}          & \multicolumn{1}{c|}{0.8199}          & \multicolumn{1}{c|}{19.2446}          & 0.1957             \\ \hline
                         & \multicolumn{1}{c|}{1}  & \multicolumn{1}{c|}{\hl{66.00\%}}  & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\hl{57.14\%}} & \multicolumn{1}{c|}{\hl{53.21\%}} & \multicolumn{1}{c|}{\hl{59.52\%}} & \multicolumn{1}{c|}{\hl{65.59\%}}  & \multicolumn{1}{c|}{\hl{60.48\%}} & \multicolumn{1}{c|}{\hl{27.2092}} & \multicolumn{1}{c|}{\hl{0.8017}} & \multicolumn{1}{c|}{\hl{18.1056}} & \hl{0.1993}    \\
                         & \multicolumn{1}{c|}{5}  & \multicolumn{1}{c|}{53.39\%}           & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}36.99\%}          & \multicolumn{1}{c|}{33.55\%}          & \multicolumn{1}{c|}{42.10\%}          & \multicolumn{1}{c|}{50.18\%}           & \multicolumn{1}{c|}{52.20\%}          & \multicolumn{1}{c|}{27.1812}          & \multicolumn{1}{c|}{0.7999}          & \multicolumn{1}{c|}{20.5338}          & 0.2032             \\
                         & \multicolumn{1}{c|}{10} & \multicolumn{1}{c|}{49.68\%}           & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}44.52\%}          & \multicolumn{1}{c|}{36.04\%}          & \multicolumn{1}{c|}{41.27\%}          & \multicolumn{1}{c|}{50.08\%}           & \multicolumn{1}{c|}{53.31\%}          & \multicolumn{1}{c|}{27.1135}          & \multicolumn{1}{c|}{0.7968}          & \multicolumn{1}{c|}{20.9897}          & 0.2049             \\
\multirow{-4}{*}{$p_1+$} & \multicolumn{1}{c|}{20} & \multicolumn{1}{c|}{51.23\%}           & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}45.71\%}          & \multicolumn{1}{c|}{35.51\%}          & \multicolumn{1}{c|}{40.87\%}          & \multicolumn{1}{c|}{49.92\%}           & \multicolumn{1}{c|}{52.88\%}          & \multicolumn{1}{c|}{27.1109}          & \multicolumn{1}{c|}{0.7967}          & \multicolumn{1}{c|}{21.2021}          & 0.2055             \\ \hline
                         & \multicolumn{1}{c|}{1}  & \multicolumn{1}{c|}{\hl{98.40\%}}  & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\hl{98.76\%}} & \multicolumn{1}{c|}{\hl{98.17\%}} & \multicolumn{1}{c|}{\hl{98.21\%}} & \multicolumn{1}{c|}{\hl{100.00\%}} & \multicolumn{1}{c|}{\hl{99.66\%}} & \multicolumn{1}{c|}{14.9437}          & \multicolumn{1}{c|}{0.4193}          & \multicolumn{1}{c|}{109.5199}         & 0.5795             \\
                         & \multicolumn{1}{c|}{5}  & \multicolumn{1}{c|}{88.57\%}           & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}90.19\%}          & \multicolumn{1}{c|}{83.12\%}          & \multicolumn{1}{c|}{82.77\%}          & \multicolumn{1}{c|}{88.87\%}           & \multicolumn{1}{c|}{83.56\%}          & \multicolumn{1}{c|}{24.286}           & \multicolumn{1}{c|}{0.7541}          & \multicolumn{1}{c|}{51.1812}          & 0.2996             \\
                         & \multicolumn{1}{c|}{10} & \multicolumn{1}{c|}{80.25\%}           & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}95.50\%}          & \multicolumn{1}{c|}{75.68\%}          & \multicolumn{1}{c|}{73.60\%}          & \multicolumn{1}{c|}{80.13\%}           & \multicolumn{1}{c|}{75.61\%}          & \multicolumn{1}{c|}{\hl{26.4921}} & \multicolumn{1}{c|}{\hl{0.797}}  & \multicolumn{1}{c|}{\hl{36.2468}} & \hl{0.2549}    \\
\multirow{-4}{*}{$p_2$}  & \multicolumn{1}{c|}{20} & \multicolumn{1}{c|}{83.09\%}           & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}96.22\%}          & \multicolumn{1}{c|}{74.64\%}          & \multicolumn{1}{c|}{76.47\%}          & \multicolumn{1}{c|}{84.32\%}           & \multicolumn{1}{c|}{76.09\%}          & \multicolumn{1}{c|}{26.4823}          & \multicolumn{1}{c|}{0.7959}          & \multicolumn{1}{c|}{36.3049}          & 0.2562             \\ \hline
                         & \multicolumn{1}{c|}{1}  & \multicolumn{1}{c|}{\hl{100.00\%}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\hl{99.38\%}} & \multicolumn{1}{c|}{\hl{97.25\%}} & \multicolumn{1}{c|}{\hl{99.40\%}} & \multicolumn{1}{c|}{\hl{100.00\%}} & \multicolumn{1}{c|}{\hl{99.66\%}} & \multicolumn{1}{c|}{13.2084}          & \multicolumn{1}{c|}{0.369}           & \multicolumn{1}{c|}{112.1609}         & 0.6103             \\
                         & \multicolumn{1}{c|}{5}  & \multicolumn{1}{c|}{90.00\%}           & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}86.46\%}          & \multicolumn{1}{c|}{85.68\%}          & \multicolumn{1}{c|}{83.84\%}          & \multicolumn{1}{c|}{90.81\%}           & \multicolumn{1}{c|}{84.70\%}          & \multicolumn{1}{c|}{22.1126}          & \multicolumn{1}{c|}{0.6987}          & \multicolumn{1}{c|}{67.3528}          & 0.3582             \\
                         & \multicolumn{1}{c|}{10} & \multicolumn{1}{c|}{76.27\%}           & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}88.95\%}          & \multicolumn{1}{c|}{72.97\%}          & \multicolumn{1}{c|}{70.71\%}          & \multicolumn{1}{c|}{79.81\%}           & \multicolumn{1}{c|}{73.17\%}          & \multicolumn{1}{c|}{24.7144}          & \multicolumn{1}{c|}{\hl{0.7628}} & \multicolumn{1}{c|}{\hl{44.6224}} & \hl{0.2906}    \\
\multirow{-4}{*}{$p_2+$} & \multicolumn{1}{c|}{20} & \multicolumn{1}{c|}{76.68\%}           & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}89.18\%}          & \multicolumn{1}{c|}{73.01\%}          & \multicolumn{1}{c|}{71.34\%}          & \multicolumn{1}{c|}{81.12\%}           & \multicolumn{1}{c|}{72.25\%}          & \multicolumn{1}{c|}{\hl{24.7179}} & \multicolumn{1}{c|}{0.7624}          & \multicolumn{1}{c|}{45.1594}          & 0.2916             \\ \hline
\end{tabular}%
}
\hfill
\resizebox{0.49\linewidth}{!}{%
\begin{tabular}{cccccccccccc}
\hline
\multicolumn{2}{c}{}                               & \multicolumn{6}{c}{neural networks}                                                                                                                                                                                                                                   & \multicolumn{4}{c}{IQAs}                                                                                       \\
\multicolumn{2}{c}{\multirow{-2}{*}{$\tau$}} & VGG19                                 & RN50                                                          & WR101                                 & DN121                                 & NNv2                                  & SNv2                                  & PSNR $\uparrow$              & SSIM $\uparrow$             & FID $\downarrow$             & LPIPS $\downarrow$ \\ \hline
                          & \multicolumn{1}{c|}{\ 1\ \ } & \multicolumn{1}{c|}{\hl{66.28\%}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}61.18\%}          & \multicolumn{1}{c|}{\hl{51.26\%}} & \multicolumn{1}{c|}{\hl{68.48\%}} & \multicolumn{1}{c|}{\hl{62.61\%}} & \multicolumn{1}{c|}{57.89\%}          & \multicolumn{1}{c|}{28.4400}   & \multicolumn{1}{c|}{0.8312} & \multicolumn{1}{c|}{13.3816} & 0.1758             \\
                          & \multicolumn{1}{c|}{2} & \multicolumn{1}{c|}{58.93\%}          & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}47.28\%}          & \multicolumn{1}{c|}{50.82\%}          & \multicolumn{1}{c|}{59.38\%}          & \multicolumn{1}{c|}{58.26\%}          & \multicolumn{1}{c|}{59.21\%}          & \multicolumn{1}{c|}{28.4669} & \multicolumn{1}{c|}{0.8315} & \multicolumn{1}{c|}{14.8572} & 0.1797             \\
                          & \multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{58.76\%}          & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\hl{69.50\%}} & \multicolumn{1}{c|}{46.67\%}          & \multicolumn{1}{c|}{49.77\%}          & \multicolumn{1}{c|}{58.80\%}          & \multicolumn{1}{c|}{\hl{60.45\%}} & \multicolumn{1}{c|}{28.2141} & \multicolumn{1}{c|}{0.8194} & \multicolumn{1}{c|}{19.1739} & 0.1964             \\
\multirow{-4}{*}{$p_1$}   & \multicolumn{1}{c|}{6} & \multicolumn{1}{c|}{56.60\%}          & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}69.08\%}          & \multicolumn{1}{c|}{42.11\%}          & \multicolumn{1}{c|}{47.72\%}          & \multicolumn{1}{c|}{54.34\%}          & \multicolumn{1}{c|}{58.77\%}          & \multicolumn{1}{c|}{28.2464} & \multicolumn{1}{c|}{0.8214} & \multicolumn{1}{c|}{18.9801} & 0.1936             \\ \hline
                          & \multicolumn{1}{c|}{1} & \multicolumn{1}{c|}{\hl{63.95\%}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\hl{58.55\%}} & \multicolumn{1}{c|}{41.18\%}          & \multicolumn{1}{c|}{\hl{64.85\%}} & \multicolumn{1}{c|}{\hl{60.08\%}} & \multicolumn{1}{c|}{\hl{60.20\%}} & \multicolumn{1}{c|}{27.2103} & \multicolumn{1}{c|}{0.8019} & \multicolumn{1}{c|}{17.4615} & 0.1981             \\
                          & \multicolumn{1}{c|}{2} & \multicolumn{1}{c|}{58.63\%}          & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}44.02\%}          & \multicolumn{1}{c|}{\hl{50.82\%}} & \multicolumn{1}{c|}{51.17\%}          & \multicolumn{1}{c|}{55.86\%}          & \multicolumn{1}{c|}{56.05\%}          & \multicolumn{1}{c|}{27.2187} & \multicolumn{1}{c|}{0.8014} & \multicolumn{1}{c|}{18.6287} & 0.2008             \\
                          & \multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{49.68\%}          & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}44.52\%}          & \multicolumn{1}{c|}{36.04\%}          & \multicolumn{1}{c|}{41.27\%}          & \multicolumn{1}{c|}{50.08\%}          & \multicolumn{1}{c|}{53.31\%}          & \multicolumn{1}{c|}{27.1135} & \multicolumn{1}{c|}{0.7968} & \multicolumn{1}{c|}{20.9897} & 0.2049             \\
\multirow{-4}{*}{$p_1+$}  & \multicolumn{1}{c|}{6} & \multicolumn{1}{c|}{50.15\%}          & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}43.71\%}          & \multicolumn{1}{c|}{31.71\%}          & \multicolumn{1}{c|}{39.60\%}          & \multicolumn{1}{c|}{48.25\%}          & \multicolumn{1}{c|}{52.47\%}          & \multicolumn{1}{c|}{27.126}  & \multicolumn{1}{c|}{0.7975} & \multicolumn{1}{c|}{20.6414} & 0.2037             \\ \hline
                          & \multicolumn{1}{c|}{1} & \multicolumn{1}{c|}{78.29\%}          & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}72.37\%}          & \multicolumn{1}{c|}{67.23\%}          & \multicolumn{1}{c|}{69.70\%}          & \multicolumn{1}{c|}{\hl{81.09\%}} & \multicolumn{1}{c|}{\hl{76.32\%}} & \multicolumn{1}{c|}{26.5986} & \multicolumn{1}{c|}{0.8032} & \multicolumn{1}{c|}{29.1863} & 0.2411             \\
                          & \multicolumn{1}{c|}{2} & \multicolumn{1}{c|}{76.19\%}          & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}67.66\%}          & \multicolumn{1}{c|}{66.67\%}          & \multicolumn{1}{c|}{70.70\%}          & \multicolumn{1}{c|}{75.08\%}          & \multicolumn{1}{c|}{75.26\%}          & \multicolumn{1}{c|}{26.6929} & \multicolumn{1}{c|}{0.8074} & \multicolumn{1}{c|}{30.2083} & 0.2377             \\
                          & \multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{\hl{80.25\%}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\hl{95.50\%}} & \multicolumn{1}{c|}{\hl{75.68\%}} & \multicolumn{1}{c|}{\hl{73.60\%}} & \multicolumn{1}{c|}{80.13\%}          & \multicolumn{1}{c|}{75.61\%}          & \multicolumn{1}{c|}{26.4921} & \multicolumn{1}{c|}{0.797}  & \multicolumn{1}{c|}{36.2468} & 0.2549             \\
\multirow{-4}{*}{$p_2$}   & \multicolumn{1}{c|}{6} & \multicolumn{1}{c|}{75.46\%}          & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}91.54\%}          & \multicolumn{1}{c|}{66.95\%}          & \multicolumn{1}{c|}{68.23\%}          & \multicolumn{1}{c|}{77.93\%}          & \multicolumn{1}{c|}{73.42\%}          & \multicolumn{1}{c|}{26.5005} & \multicolumn{1}{c|}{0.798}  & \multicolumn{1}{c|}{35.1451} & 0.2523             \\ \hline
                          & \multicolumn{1}{c|}{1} & \multicolumn{1}{c|}{73.26\%}          & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}72.37\%}          & \multicolumn{1}{c|}{67.23\%}          & \multicolumn{1}{c|}{\hl{75.76\%}} & \multicolumn{1}{c|}{\hl{81.09\%}} & \multicolumn{1}{c|}{72.04\%}          & \multicolumn{1}{c|}{24.7843} & \multicolumn{1}{c|}{0.7682} & \multicolumn{1}{c|}{39.6818} & 0.2812             \\
                          & \multicolumn{1}{c|}{2} & \multicolumn{1}{c|}{73.51\%}          & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}61.14\%}          & \multicolumn{1}{c|}{64.48\%}          & \multicolumn{1}{c|}{69.14\%}          & \multicolumn{1}{c|}{80.78\%}          & \multicolumn{1}{c|}{68.16\%}          & \multicolumn{1}{c|}{24.8393} & \multicolumn{1}{c|}{0.7702} & \multicolumn{1}{c|}{40.8266} & 0.2797             \\
                          & \multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{\hl{76.27\%}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\hl{88.95\%}} & \multicolumn{1}{c|}{\hl{72.97\%}} & \multicolumn{1}{c|}{70.71\%}          & \multicolumn{1}{c|}{79.81\%}          & \multicolumn{1}{c|}{\hl{73.17\%}} & \multicolumn{1}{c|}{24.7144} & \multicolumn{1}{c|}{0.7628} & \multicolumn{1}{c|}{44.6224} & 0.2906             \\
\multirow{-4}{*}{$p_2+$}  & \multicolumn{1}{c|}{6} & \multicolumn{1}{c|}{73.31\%}          & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}78.95\%}          & \multicolumn{1}{c|}{65.27\%}          & \multicolumn{1}{c|}{65.10\%}          & \multicolumn{1}{c|}{78.08\%}          & \multicolumn{1}{c|}{68.31\%}          & \multicolumn{1}{c|}{24.7084} & \multicolumn{1}{c|}{0.7636} & \multicolumn{1}{c|}{44.5897} & 0.2889             \\ \hline
\end{tabular}%
}
\caption{Ablation study on $\epsilon$, $I$, $L$, and $\tau$.}
\end{table*}

==> sdxl-asr-iqa.tex <==
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccccccc}
\hline
\multicolumn{2}{c}{}                                                                & \multicolumn{6}{c}{neural networks}                                                                                                                                                                             & \multicolumn{4}{c}{IQAs}                                                                                                                  \\
\multicolumn{2}{c}{\multirow{-2}{*}{attack methods}}                                & VGG19                        & RN50                                                 & WR101                        & DN121                        & NNv2                         & SNv2                         & PSNR $\uparrow$                       & SSIM $\uparrow$                      & FID $\downarrow$                      & LPIPS $\downarrow$ \\ \hline
\multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{SDXL-PGD}       & \multicolumn{1}{c|}{52.47\%} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}53.59\%} & \multicolumn{1}{c|}{38.33\%} & \multicolumn{1}{c|}{46.35\%} & \multicolumn{1}{c|}{52.99\%} & \multicolumn{1}{c|}{58.61\%} & \multicolumn{1}{c|}{28.3105}          & \multicolumn{1}{c|}{0.8263}          & \multicolumn{1}{c|}{16.2421}          & 0.1847             \\
\multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{SDXL-Turbo-PGD} & \multicolumn{1}{c|}{57.33\%} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}54.88\%} & \multicolumn{1}{c|}{45.35\%} & \multicolumn{1}{c|}{51.54\%} & \multicolumn{1}{c|}{59.17\%} & \multicolumn{1}{c|}{57.90\%} & \multicolumn{1}{c|}{28.2142}          & \multicolumn{1}{c|}{0.8197}          & \multicolumn{1}{c|}{\hl{17.2365}} & \hl{0.1926}    \\
\multicolumn{1}{c|}{\multirow{-3}{*}{$p_1$}}  & \multicolumn{1}{c|}{Diff-PGD}       & \multicolumn{1}{c|}{55.47\%} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}78.98\%} & \multicolumn{1}{c|}{39.43\%} & \multicolumn{1}{c|}{44.88\%} & \multicolumn{1}{c|}{56.16\%} & \multicolumn{1}{c|}{55.86\%} & \multicolumn{1}{c|}{\hl{28.3815}} & \multicolumn{1}{c|}{\hl{0.8293}} & \multicolumn{1}{c|}{17.1181}          & 0.1842             \\ \hline
\multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{SDXL-PGD}       & \multicolumn{1}{c|}{64.35\%} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}38.42\%} & \multicolumn{1}{c|}{48.02\%} & \multicolumn{1}{c|}{53.47\%} & \multicolumn{1}{c|}{65.67\%} & \multicolumn{1}{c|}{74.85\%} & \multicolumn{1}{c|}{22.8103}          & \multicolumn{1}{c|}{0.5659}          & \multicolumn{1}{c|}{37.5139}          & 0.3615             \\
\multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{SDXL-Turbo-PGD} & \multicolumn{1}{c|}{70.50\%} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}42.45\%} & \multicolumn{1}{c|}{51.55\%} & \multicolumn{1}{c|}{58.77\%} & \multicolumn{1}{c|}{68.24\%} & \multicolumn{1}{c|}{74.82\%} & \multicolumn{1}{c|}{22.6434}          & \multicolumn{1}{c|}{0.5487}          & \multicolumn{1}{c|}{39.5332}          & 0.3749             \\
\multicolumn{1}{c|}{\multirow{-3}{*}{$p_1+$}} & \multicolumn{1}{c|}{Diff-PGD}       & \multicolumn{1}{c|}{49.11\%} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}46.05\%} & \multicolumn{1}{c|}{27.57\%} & \multicolumn{1}{c|}{37.34\%} & \multicolumn{1}{c|}{44.28\%} & \multicolumn{1}{c|}{50.00\%} & \multicolumn{1}{c|}{\hl{27.1843}} & \multicolumn{1}{c|}{\hl{0.8013}} & \multicolumn{1}{c|}{\hl{19.4638}} & \hl{0.2013}    \\ \hline
\end{tabular}%
}

==> tab-asr-iqa.tex <==
\resizebox{0.95\textwidth}{!}{%
\begin{tabular}{ccccccccccccc}
\hline
                                               & \multicolumn{2}{c}{}                                                          & \multicolumn{6}{c}{neural networks}                                                                                                                                                                                                                                                                                   & \multicolumn{4}{c}{IQAs}                                                                                       \\
\multirow{-2}{*}{white-box models}             & \multicolumn{2}{c}{\multirow{-2}{*}{attack methods}}                          & VGG19                                 & RN50                                                          & WR101                                                         & DN121                                                         & NNv2                                  & SNv2                                  & PSNR $\uparrow$              & SSIM $\uparrow$             & FID $\downarrow$             & LPIPS $\downarrow$ \\ \hline
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{PGD}      & \multicolumn{1}{c|}{50.39\%}          & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}35.37\%}          & \multicolumn{1}{c|}{30.82\%}                                  & \multicolumn{1}{c|}{39.71\%}                                  & \multicolumn{1}{c|}{47.33\%}          & \multicolumn{1}{c|}{51.43\%}          & \multicolumn{1}{c|}{28.5391} & \multicolumn{1}{c|}{0.8370} & \multicolumn{1}{c|}{14.9556} & 0.1738             \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{Diff-PGD} & \multicolumn{1}{c|}{55.47\%}          & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\hl{78.98\%}} & \multicolumn{1}{c|}{39.43\%}                                  & \multicolumn{1}{c|}{44.88\%}                                  & \multicolumn{1}{c|}{56.16\%}          & \multicolumn{1}{c|}{55.86\%}          & \multicolumn{1}{c|}{28.3815} & \multicolumn{1}{c|}{0.8293} & \multicolumn{1}{c|}{17.1181} & 0.1842             \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{\multirow{-3}{*}{$p_1$}}  & \multicolumn{1}{c|}{Ours}     & \multicolumn{1}{c|}{\hl{58.76\%}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}69.50\%}          & \multicolumn{1}{c|}{\hl{46.67\%}}                         & \multicolumn{1}{c|}{\hl{49.77\%}}                         & \multicolumn{1}{c|}{\hl{58.80\%}} & \multicolumn{1}{c|}{\hl{60.45\%}} & \multicolumn{1}{c|}{28.2141} & \multicolumn{1}{c|}{0.8194} & \multicolumn{1}{c|}{19.1739} & 0.1964             \\ \cline{2-13} 
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{PGD}      & \multicolumn{1}{c|}{46.85\%}          & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}23.85\%}          & \multicolumn{1}{c|}{26.03\%}                                  & \multicolumn{1}{c|}{35.06\%}                                  & \multicolumn{1}{c|}{45.42\%}          & \multicolumn{1}{c|}{49.18\%}          & \multicolumn{1}{c|}{27.2513} & \multicolumn{1}{c|}{0.8041} & \multicolumn{1}{c|}{18.9602} & 0.1990             \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{Diff-PGD} & \multicolumn{1}{c|}{49.11\%}          & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\hl{46.05\%}} & \multicolumn{1}{c|}{27.57\%}                                  & \multicolumn{1}{c|}{37.34\%}                                  & \multicolumn{1}{c|}{44.28\%}          & \multicolumn{1}{c|}{50.00\%}          & \multicolumn{1}{c|}{27.1843} & \multicolumn{1}{c|}{0.8013} & \multicolumn{1}{c|}{19.4638} & 0.2013             \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{\multirow{-3}{*}{$p_1+$}} & \multicolumn{1}{c|}{Ours}     & \multicolumn{1}{c|}{\hl{49.68\%}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}44.52\%}          & \multicolumn{1}{c|}{\hl{36.04\%}}                         & \multicolumn{1}{c|}{\hl{41.27\%}}                         & \multicolumn{1}{c|}{\hl{50.08\%}} & \multicolumn{1}{c|}{\hl{53.31\%}} & \multicolumn{1}{c|}{27.1135} & \multicolumn{1}{c|}{0.7968} & \multicolumn{1}{c|}{20.9897} & 0.2049             \\ \cline{2-13} 
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{PGD}      & \multicolumn{1}{c|}{64.57\%}          & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}43.49\%}          & \multicolumn{1}{c|}{48.17\%}                                  & \multicolumn{1}{c|}{49.37\%}                                  & \multicolumn{1}{c|}{65.65\%}          & \multicolumn{1}{c|}{64.75\%}          & \multicolumn{1}{c|}{26.7452} & \multicolumn{1}{c|}{0.8125} & \multicolumn{1}{c|}{29.1990} & 0.2280             \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{Diff-PGD} & \multicolumn{1}{c|}{66.42\%}          & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}68.27\%}          & \multicolumn{1}{c|}{47.14\%}                                  & \multicolumn{1}{c|}{55.12\%}                                  & \multicolumn{1}{c|}{67.16\%}          & \multicolumn{1}{c|}{67.43\%}          & \multicolumn{1}{c|}{26.5719} & \multicolumn{1}{c|}{0.8036} & \multicolumn{1}{c|}{31.5850} & 0.2415             \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{\multirow{-3}{*}{$p_2$}}  & \multicolumn{1}{c|}{Ours}     & \multicolumn{1}{c|}{\hl{80.25\%}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\hl{95.50\%}} & \multicolumn{1}{c|}{\hl{75.68\%}}                         & \multicolumn{1}{c|}{\hl{73.60\%}}                         & \multicolumn{1}{c|}{\hl{80.13\%}} & \multicolumn{1}{c|}{\hl{75.61\%}} & \multicolumn{1}{c|}{26.4921} & \multicolumn{1}{c|}{0.7970} & \multicolumn{1}{c|}{36.2468} & 0.2549             \\ \cline{2-13} 
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{PGD}      & \multicolumn{1}{c|}{65.35\%}          & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}42.38\%}          & \multicolumn{1}{c|}{53.20\%}                                  & \multicolumn{1}{c|}{56.17\%}                                  & \multicolumn{1}{c|}{71.76\%}          & \multicolumn{1}{c|}{60.66\%}          & \multicolumn{1}{c|}{24.8956} & \multicolumn{1}{c|}{0.7744} & \multicolumn{1}{c|}{38.6395} & 0.2715             \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{Diff-PGD} & \multicolumn{1}{c|}{65.38\%}          & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}56.06\%}          & \multicolumn{1}{c|}{51.86\%}                                  & \multicolumn{1}{c|}{55.63\%}                                  & \multicolumn{1}{c|}{69.65\%}          & \multicolumn{1}{c|}{63.36\%}          & \multicolumn{1}{c|}{24.7742} & \multicolumn{1}{c|}{0.7678} & \multicolumn{1}{c|}{41.6833} & 0.2811             \\
\multicolumn{1}{c|}{\multirow{-12}{*}{RN50}}   & \multicolumn{1}{c|}{\multirow{-3}{*}{$p_2+$}} & \multicolumn{1}{c|}{Ours}     & \multicolumn{1}{c|}{\hl{76.27\%}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\hl{88.95\%}} & \multicolumn{1}{c|}{\hl{72.97\%}}                         & \multicolumn{1}{c|}{\hl{70.71\%}}                         & \multicolumn{1}{c|}{\hl{79.81\%}} & \multicolumn{1}{c|}{\hl{73.17\%}} & \multicolumn{1}{c|}{24.7144} & \multicolumn{1}{c|}{0.7628} & \multicolumn{1}{c|}{44.6224} & 0.2906             \\ \hline
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{PGD}      & \multicolumn{1}{c|}{51.92\%}          & \multicolumn{1}{c|}{36.17\%}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}34.67\%}          & \multicolumn{1}{c|}{41.14\%}                                  & \multicolumn{1}{c|}{50.31\%}          & \multicolumn{1}{c|}{57.39\%}          & \multicolumn{1}{c|}{28.5138} & \multicolumn{1}{c|}{0.8353} & \multicolumn{1}{c|}{14.8201} & 0.1754             \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{Diff-PGD} & \multicolumn{1}{c|}{55.83\%}          & \multicolumn{1}{c|}{44.81\%}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\hl{75.53\%}} & \multicolumn{1}{c|}{49.92\%}                                  & \multicolumn{1}{c|}{57.27\%}          & \multicolumn{1}{c|}{58.33\%}          & \multicolumn{1}{c|}{28.3655} & \multicolumn{1}{c|}{0.8280} & \multicolumn{1}{c|}{16.7484} & 0.1853             \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{\multirow{-3}{*}{$p_1$}}  & \multicolumn{1}{c|}{Ours}     & \multicolumn{1}{c|}{\hl{61.39\%}} & \multicolumn{1}{c|}{\hl{50.66\%}}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}62.39\%}          & \multicolumn{1}{c|}{\hl{51.24\%}}                         & \multicolumn{1}{c|}{\hl{59.39\%}} & \multicolumn{1}{c|}{\hl{58.96\%}} & \multicolumn{1}{c|}{28.1855} & \multicolumn{1}{c|}{0.8173} & \multicolumn{1}{c|}{19.0033} & 0.1983             \\ \cline{2-13} 
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{PGD}      & \multicolumn{1}{c|}{46.37\%}          & \multicolumn{1}{c|}{32.01\%}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}20.04\%}          & \multicolumn{1}{c|}{38.90\%}                                  & \multicolumn{1}{c|}{44.44\%}          & \multicolumn{1}{c|}{\hl{56.09\%}} & \multicolumn{1}{c|}{27.2350} & \multicolumn{1}{c|}{0.8033} & \multicolumn{1}{c|}{18.6536} & 0.1993             \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{Diff-PGD} & \multicolumn{1}{c|}{47.48\%}          & \multicolumn{1}{c|}{36.31\%}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\hl{41.52\%}} & \multicolumn{1}{c|}{38.33\%}                                  & \multicolumn{1}{c|}{46.71\%}          & \multicolumn{1}{c|}{52.59\%}          & \multicolumn{1}{c|}{27.1764} & \multicolumn{1}{c|}{0.8007} & \multicolumn{1}{c|}{19.3679} & 0.2016             \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{\multirow{-3}{*}{$p_1+$}} & \multicolumn{1}{c|}{Ours}     & \multicolumn{1}{c|}{\hl{54.24\%}} & \multicolumn{1}{c|}{\hl{39.60\%}}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}39.18\%}          & \multicolumn{1}{c|}{\hl{39.93\%}}                         & \multicolumn{1}{c|}{\hl{51.26\%}} & \multicolumn{1}{c|}{53.73\%}          & \multicolumn{1}{c|}{27.0974} & \multicolumn{1}{c|}{0.7956} & \multicolumn{1}{c|}{20.6378} & 0.2065             \\ \cline{2-13} 
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{PGD}      & \multicolumn{1}{c|}{66.03\%}          & \multicolumn{1}{c|}{48.46\%}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}39.08\%}          & \multicolumn{1}{c|}{52.34\%}                                  & \multicolumn{1}{c|}{65.20\%}          & \multicolumn{1}{c|}{64.35\%}          & \multicolumn{1}{c|}{26.7511} & \multicolumn{1}{c|}{0.8125} & \multicolumn{1}{c|}{28.7923} & 0.2289             \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{Diff-PGD} & \multicolumn{1}{c|}{68.70\%}          & \multicolumn{1}{c|}{54.18\%}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}62.29\%}          & \multicolumn{1}{c|}{56.26\%}                                  & \multicolumn{1}{c|}{67.65\%}          & \multicolumn{1}{c|}{68.89\%}          & \multicolumn{1}{c|}{26.5408} & \multicolumn{1}{c|}{0.8027} & \multicolumn{1}{c|}{31.5989} & 0.2434             \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{\multirow{-3}{*}{$p_2$}}  & \multicolumn{1}{c|}{Ours}     & \multicolumn{1}{c|}{\hl{80.60\%}} & \multicolumn{1}{c|}{\hl{74.59\%}}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\hl{95.80\%}} & \multicolumn{1}{c|}{\hl{71.91\%}}                         & \multicolumn{1}{c|}{\hl{82.67\%}} & \multicolumn{1}{c|}{\hl{78.36\%}} & \multicolumn{1}{c|}{26.4814} & \multicolumn{1}{c|}{0.7970} & \multicolumn{1}{c|}{35.1437} & 0.2528             \\ \cline{2-13} 
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{PGD}      & \multicolumn{1}{c|}{63.68\%}          & \multicolumn{1}{c|}{53.16\%}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}39.18\%}          & \multicolumn{1}{c|}{54.18\%}                                  & \multicolumn{1}{c|}{70.44\%}          & \multicolumn{1}{c|}{62.39\%}          & \multicolumn{1}{c|}{24.9099} & \multicolumn{1}{c|}{0.7749} & \multicolumn{1}{c|}{38.1896} & 0.2714             \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{Diff-PGD} & \multicolumn{1}{c|}{69.22\%}          & \multicolumn{1}{c|}{56.05\%}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}50.05\%}          & \multicolumn{1}{c|}{59.66\%}                                  & \multicolumn{1}{c|}{70.76\%}          & \multicolumn{1}{c|}{62.78\%}          & \multicolumn{1}{c|}{24.7410} & \multicolumn{1}{c|}{0.7667} & \multicolumn{1}{c|}{41.8474} & 0.2831             \\
\multicolumn{1}{c|}{\multirow{-12}{*}{WRN101}} & \multicolumn{1}{c|}{\multirow{-3}{*}{$p_2+$}} & \multicolumn{1}{c|}{Ours}     & \multicolumn{1}{c|}{\hl{75.33\%}} & \multicolumn{1}{c|}{\hl{72.28\%}}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\hl{86.03\%}} & \multicolumn{1}{c|}{\hl{70.85\%}}                         & \multicolumn{1}{c|}{\hl{81.77\%}} & \multicolumn{1}{c|}{\hl{72.57\%}} & \multicolumn{1}{c|}{24.7115} & \multicolumn{1}{c|}{0.7633} & \multicolumn{1}{c|}{43.9790} & 0.2887             \\ \hline
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{PGD}      & \multicolumn{1}{c|}{46.92\%}          & \multicolumn{1}{c|}{35.62\%}                                  & \multicolumn{1}{c|}{32.59\%}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}52.00\%}          & \multicolumn{1}{c|}{45.16\%}          & \multicolumn{1}{c|}{52.77\%}          & \multicolumn{1}{c|}{28.5101} & \multicolumn{1}{c|}{0.8358} & \multicolumn{1}{c|}{15.4706} & 0.1751             \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{Diff-PGD} & \multicolumn{1}{c|}{55.95\%}          & \multicolumn{1}{c|}{46.84\%}                                  & \multicolumn{1}{c|}{41.76\%}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\hl{89.80\%}} & \multicolumn{1}{c|}{55.65\%}          & \multicolumn{1}{c|}{57.47\%}          & \multicolumn{1}{c|}{28.3412} & \multicolumn{1}{c|}{0.8286} & \multicolumn{1}{c|}{18.5986} & 0.1860             \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{\multirow{-3}{*}{$p_1$}}  & \multicolumn{1}{c|}{Ours}     & \multicolumn{1}{c|}{\hl{60.64\%}} & \multicolumn{1}{c|}{\hl{52.52\%}}                         & \multicolumn{1}{c|}{\hl{48.85\%}}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}77.79\%}          & \multicolumn{1}{c|}{\hl{56.60\%}} & \multicolumn{1}{c|}{\hl{59.04\%}} & \multicolumn{1}{c|}{28.1799} & \multicolumn{1}{c|}{0.8189} & \multicolumn{1}{c|}{20.7998} & 0.1988             \\ \cline{2-13} 
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{PGD}      & \multicolumn{1}{c|}{45.52\%}          & \multicolumn{1}{c|}{32.11\%}                                  & \multicolumn{1}{c|}{30.82\%}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}33.50\%}          & \multicolumn{1}{c|}{42.53\%}          & \multicolumn{1}{c|}{49.82\%}          & \multicolumn{1}{c|}{27.2361} & \multicolumn{1}{c|}{0.8032} & \multicolumn{1}{c|}{19.3294} & 0.1994             \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{Diff-PGD} & \multicolumn{1}{c|}{46.37\%}          & \multicolumn{1}{c|}{34.18\%}                                  & \multicolumn{1}{c|}{30.30\%}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\hl{59.60\%}} & \multicolumn{1}{c|}{45.33\%}          & \multicolumn{1}{c|}{52.29\%}          & \multicolumn{1}{c|}{27.1603} & \multicolumn{1}{c|}{0.8001} & \multicolumn{1}{c|}{20.1820} & 0.2024             \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{\multirow{-3}{*}{$p_1+$}} & \multicolumn{1}{c|}{Ours}     & \multicolumn{1}{c|}{\hl{52.58\%}} & \multicolumn{1}{c|}{\hl{42.90\%}}                         & \multicolumn{1}{c|}{\hl{39.50\%}}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}56.58\%}          & \multicolumn{1}{c|}{\hl{50.46\%}} & \multicolumn{1}{c|}{\hl{54.06\%}} & \multicolumn{1}{c|}{27.0858} & \multicolumn{1}{c|}{0.7954} & \multicolumn{1}{c|}{21.5762} & 0.2072             \\ \cline{2-13} 
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{PGD}      & \multicolumn{1}{c|}{62.74\%}          & \multicolumn{1}{c|}{50.16\%}                                  & \multicolumn{1}{c|}{52.11\%}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}54.70\%}          & \multicolumn{1}{c|}{60.92\%}          & \multicolumn{1}{c|}{63.10\%}          & \multicolumn{1}{c|}{26.7231} & \multicolumn{1}{c|}{0.8121} & \multicolumn{1}{c|}{29.6638} & 0.2282             \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{Diff-PGD} & \multicolumn{1}{c|}{63.20\%}          & \multicolumn{1}{c|}{52.91\%}                                  & \multicolumn{1}{c|}{51.96\%}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}81.50\%}          & \multicolumn{1}{c|}{65.27\%}          & \multicolumn{1}{c|}{65.40\%}          & \multicolumn{1}{c|}{26.5851} & \multicolumn{1}{c|}{0.8046} & \multicolumn{1}{c|}{32.5457} & 0.2408             \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{\multirow{-3}{*}{$p_2$}}  & \multicolumn{1}{c|}{Ours}     & \multicolumn{1}{c|}{\hl{79.79\%}} & \multicolumn{1}{c|}{\hl{73.59\%}}                         & \multicolumn{1}{c|}{\hl{73.28\%}}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\hl{96.48\%}} & \multicolumn{1}{c|}{\hl{78.99\%}} & \multicolumn{1}{c|}{\hl{75.95\%}} & \multicolumn{1}{c|}{26.5331} & \multicolumn{1}{c|}{0.7990} & \multicolumn{1}{c|}{36.4909} & 0.2514             \\ \cline{2-13} 
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{PGD}      & \multicolumn{1}{c|}{63.44\%}          & \multicolumn{1}{c|}{55.11\%}                                  & \multicolumn{1}{c|}{54.77\%}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}50.40\%}          & \multicolumn{1}{c|}{66.34\%}          & \multicolumn{1}{c|}{61.44\%}          & \multicolumn{1}{c|}{24.8592} & \multicolumn{1}{c|}{0.7740} & \multicolumn{1}{c|}{39.6970} & 0.2698             \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{Diff-PGD} & \multicolumn{1}{c|}{62.11\%}          & \multicolumn{1}{c|}{54.68\%}                                  & \multicolumn{1}{c|}{53.85\%}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}63.20\%}          & \multicolumn{1}{c|}{69.74\%}          & \multicolumn{1}{c|}{61.59\%}          & \multicolumn{1}{c|}{24.7774} & \multicolumn{1}{c|}{0.7688} & \multicolumn{1}{c|}{42.3275} & 0.2779             \\
\multicolumn{1}{c|}{\multirow{-12}{*}{DN121}}  & \multicolumn{1}{c|}{\multirow{-3}{*}{$p_2+$}} & \multicolumn{1}{c|}{Ours}     & \multicolumn{1}{c|}{\hl{75.08\%}} & \multicolumn{1}{c|}{\hl{70.08\%}}                         & \multicolumn{1}{c|}{\hl{66.60\%}}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\hl{88.84\%}} & \multicolumn{1}{c|}{\hl{78.37\%}} & \multicolumn{1}{c|}{\hl{70.65\%}} & \multicolumn{1}{c|}{24.7393} & \multicolumn{1}{c|}{0.7646} & \multicolumn{1}{c|}{46.0230} & 0.2857             \\ \hline
\end{tabular}%
}
